Equilibrium-Invariant Embedding, Metric Space, and Fundamental Set of $2\times2$ Normal-Form Games

Equilibrium solution concepts of normal-form games, such as Nash equilibria, correlated equilibria, and coarse correlated equilibria, describe the joint strategy profiles from which no player has incentive to unilaterally deviate. They are widely studied in game theory, economics, and multiagent systems. Equilibrium concepts are invariant under certain transforms of the payoffs. We define an equilibrium-inspired distance metric for the space of all normal-form games and uncover a distance-preserving equilibrium-invariant embedding. Furthermore, we propose an additional transform which defines a better-response-invariant distance metric and embedding. To demonstrate these metric spaces we study $2\times2$ games. The equilibrium-invariant embedding of $2\times2$ games has an efficient two variable parameterization (a reduction from eight), where each variable geometrically describes an angle on a unit circle. Interesting properties can be spatially inferred from the embedding, including: equilibrium support, cycles, competition, coordination, distances, best-responses, and symmetries. The best-response-invariant embedding of $2\times2$ games, after considering symmetries, rediscovers a set of 15 games, and their respective equivalence classes. We propose that this set of game classes is fundamental and captures all possible interesting strategic interactions in $2\times2$ games. We introduce a directed graph representation and name for each class. Finally, we leverage the tools developed for $2\times2$ games to develop game theoretic visualizations of large normal-form and extensive-form games that aim to fingerprint the strategic interactions that occur within.

==> old/part_game_names_old.tex <==
% Games.
\node[label={[align=left]-45:{\tiny \coordinationgame Coordination \coordinationsupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,0.5) {};
\node[label={-45:{\tiny \fossickgame Fossick \fossicksupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.25,0.25) {};
\node[label={[align=right]135:{\tiny \dominantgame Dominant \dominantsupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.0,0.0) {};
\node[label={-45:{\tiny \daredevilgame Daredevil \daredevilsupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:-0.25,-0.25) {};
\node[label={[align=left]45:{\tiny \cyclegame Cycle \cyclesupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,-0.5) {};

\node[label={-45:{\tiny \aidosgame Aidos \aidossupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.0,-0.25) {};
\node[label={45:{\tiny \heistgame Heist \heistsupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.25,-0.25) {};
\node[label={-45:{\tiny \hazardgame Hazard \hazardsupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,-0.25) {};
\node[label={-45:{\tiny \picnicgame Picnic \picnicsupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.25,0.0) {};
\node[label={-45:{\tiny \samaritangame Samaritan \samaritansupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,0.0) {};
\node[label={-45:{\tiny \safetygame Safety \safetysupport}},circle,draw,inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,0.25) {};


==> tex/figure_equivariant_basins.tex <==
\begin{tikzpicture}[
    /pgfplots/y=7cm, /pgfplots/x=7cm, % To make sure all the plots use the same scale
    % remember picture,
    % transform shape,
    % myscalar,
]
\begin{axis}[
    % width=16cm,height=16cm,
    anchor=origin, % Shift the axis so its origin is at (0,0)
    axis lines = middle,
    xmin=-1.1, xmax=+1.1,
    ymin=-1.1, ymax=+1.1,
    xticklabels={,\(+\pi\)}, xtick={-1,+1},
    yticklabels={,\(+\pi\)}, ytick={-1,+1},
    xlabel = \(\theta_1\),
    ylabel = {\(\theta_2\)},
        xmajorgrids=true,
        ymajorgrids=true,
    grid style=dashed,
]

\input{tex/part_equilibrium_boundaries}
% \input{tex/part_quadrant_names}

\end{axis}

\begin{pgfinterruptboundingbox}
    \foreach \x / \width / \xa / \xb in {
        -1.0 / 29mm /-1/-1,
        -0.75 / 6mm /-1/0,
        -0.5 / 29mm /-1/1,
        -0.25 / 6mm /0/1,
        0.0 / 29mm /1/1,
        0.25 / 6mm /1/0,
        0.5 / 29mm /1/-1,
        0.75 / 6mm /0/-1,
        1.0 / 29mm /-1/-1}
        {
        \foreach \y / \height / \ya / \yb in {
            -1.0 / 29mm /-1/-1,
            -0.75 / 6mm /-1/0,
            -0.5 / 29mm /-1/1,
            -0.25 / 6mm /0/1,
            0.0 / 29mm /1/1,
            0.25 / 6mm /1/0,
            0.5 / 29mm /1/-1,
            0.75 / 6mm /0/-1,
            1.0 / 29mm /-1/-1}
            {
                \ifthenelse{\equal{\width}{\height}}{
                    \node[] at (\x * 7cm,\y * 7cm) [rectangle,draw,minimum width=\width,minimum height=\height,dotted] {};
                }{}
                \node[] at (\x * 7cm,\y * 7cm) [] {\equigame{\xa}{\xb}{\ya}{\yb}};
            }
        }
            
    \fill [white] (-9cm,-9cm) rectangle (-7.7cm,9cm);
    \fill [white] (-9cm,-9cm) rectangle (9cm,-7.7cm);
    \fill [white] (7.7cm,-9cm) rectangle (9cm,9cm);
    \fill [white] (-9cm,7.7cm) rectangle (9cm,9cm);
\end{pgfinterruptboundingbox}

\begin{axis}[
    x=7cm,
    y=7cm,
    anchor={7.7cm,9.5cm}, % Shift the axis so its origin is at (0,0)
    axis lines = middle,
    xmin=-1.1, xmax=+1.1,
    ymin=-0.1, ymax=+0.1,
    xticklabels={\(-\pi\),\(+\pi\)}, xtick={-1,1},
    xlabel = \(\theta_1\),
    axis y line=none,
    xmajorgrids=true,
    grid style=dashed,
]
\end{axis}

\begin{pgfinterruptboundingbox}
    \foreach \x / \width / \xa / \xb in {
        -1.0 / 29mm /-1/-1,
        -0.75 / 6mm /-1/0,
        -0.5 / 29mm /-1/1,
        -0.25 / 6mm /0/1,
        0.0 / 29mm /1/1,
        0.25 / 6mm /1/0,
        0.5 / 29mm /1/-1,
        0.75 / 6mm /0/-1,
        1.0 / 29mm /-1/-1}
        {
            \node[] at (\x * 7cm,-8.8cm) [rectangle,draw,minimum width=\width,minimum height=6mm,dotted] {};
            \node[] at (\x * 7cm,-8.8cm) [] {\equigame{\xa}{\xb}{0}{0}};
        }

    \fill [white] (7.7cm,-10cm) rectangle (9cm,-8cm);
    \fill [white] (-9cm,-10cm) rectangle (-7.7,-8cm);
\end{pgfinterruptboundingbox}

\begin{axis}[
    x=7cm,
    y=7cm,
    anchor={9.5cm,7.7cm}, % Shift the axis so its origin is at (0,0)
    axis lines = middle,
    xmin=-0.1, xmax=+0.1,
    ymin=-1.1, ymax=+1.1,
    yticklabels={\(-\pi\),\(+\pi\)}, ytick={-1,1},
    ylabel = \(\theta_2\),
    axis x line=none,
    ymajorgrids=true,
    grid style=dashed,
]
\end{axis}

\begin{pgfinterruptboundingbox}
    \foreach \y / \height / \ya / \yb in {
        -1.0 / 29mm /-1/-1,
        -0.75 / 6mm /-1/0,
        -0.5 / 29mm /-1/1,
        -0.25 / 6mm /0/1,
        0.0 / 29mm /1/1,
        0.25 / 6mm /1/0,
        0.5 / 29mm /1/-1,
        0.75 / 6mm /0/-1,
        1.0 / 29mm /-1/-1}
        {
            \node[] at (-8.8cm,\y * 7cm) [rectangle,draw,minimum width=6mm,minimum height=\height,dotted] {};
            \node[] at (-8.8cm,\y * 7cm) [] {\equigame{0}{0}{\ya}{\yb}};
        }

    \fill [white] (-10cm,7.7cm) rectangle (-8cm,9cm);
    \fill [white] (-10cm,-9cm) rectangle (-8cm,-7.7);
\end{pgfinterruptboundingbox}


\begin{pgfinterruptboundingbox}
    \node[] at (-8.8cm,-8.8cm) [] {\equigame{0}{0}{0}{0}};
\end{pgfinterruptboundingbox}

\end{tikzpicture}

==> tex/part_equilibrium_boundaries.tex <==
% Stag Hunt Equilibrium.
\addplot+[
    only marks,
    mark=*,
    mark options={solid},
    mark size=0.75pt,
    color=gray]
coordinates {(0.25,0.25) (0.75,0.75) (-0.25,-0.75) (-0.75,-0.25)};

% Left equilibrium.
\addplot[color=gray] coordinates {(-0.25,0.73) (-0.25,-0.23)};
\addplot[color=gray] coordinates {(0.75,0.23) (0.75,-0.73)};

% Top equilibrium.
\addplot[color=gray] coordinates {(-0.73,0.75) (0.23,0.75)};
\addplot[color=gray] coordinates {(-0.23,-0.25) (0.73,-0.25)};

% Right equilibrium.
\addplot[color=gray] coordinates {(0.25,1.0) (0.25,0.77)};
\addplot[color=gray] coordinates {(0.25,-0.27) (0.25,-1.0)};
\addplot[color=gray] coordinates {(-0.75,1.0) (-0.75,0.27)};
\addplot[color=gray] coordinates {(-0.75,-0.77) (-0.75,-1.0)};

% Bottom equilibrium.
\addplot[color=gray] coordinates {(-1.0,0.25) (-0.27,0.25)};
\addplot[color=gray] coordinates {(0.77,0.25) (1.0,0.25)};
\addplot[color=gray] coordinates {(-1.0,-0.75) (-0.77,-0.75)};
\addplot[color=gray] coordinates {(0.27,-0.75) (1.0,-0.75)};

% Three-equilibrium.
\addplot[color=gray] coordinates {(0.25,0.27) (0.25,0.75) (0.73,0.75)};
\addplot[color=gray] coordinates {(0.27,0.25) (0.75,0.25) (0.75,0.73)};

\addplot[color=gray] coordinates {(-0.75,-0.27) (-0.75,-0.75) (-0.27,-0.75)};
\addplot[color=gray] coordinates {(-0.73,-0.25) (-0.25,-0.25) (-0.25,-0.73)};


==> tex/part_game_names.tex <==
% Games.
\node[label={[align=left]-45:{\tiny Coordination}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,0.5) {};
\node[label={-45:{\tiny Fossick}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.25,0.25) {};
\node[label={[align=right]135:{\tiny Dominant}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.0,0.0) {};
\node[label={-45:{\tiny Daredevil}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:-0.25,-0.25) {};
\node[label={[align=left]45:{\tiny Cycle}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,-0.5) {};

\node[label={-45:{\tiny Aidos}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.0,-0.25) {};
\node[label={45:{\tiny Heist}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.25,-0.25) {};
\node[label={-45:{\tiny Hazard}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,-0.25) {};
\node[label={-45:{\tiny Picnic}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.25,0.0) {};
\node[label={-45:{\tiny Samaritan}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,0.0) {};
\node[label={-45:{\tiny Safety}},inner sep=1pt,minimum size=1pt,line width=0.2pt] at (axis cs:0.5,0.25) {};


==> tex/part_player_permutation.tex <==
% Permutations.
\addplot[dashed,color=gray] coordinates {(-1.1,-1.1)(1.1,1.1)};
\addplot[dashed,color=gray] coordinates {(0.5, 1.1)(0.5, -1.1)};
\addplot[dashed,color=gray] coordinates {(-0.5, 1.1)(-0.5, -1.1)};
\addplot[dashed,color=gray] coordinates {(1.1, 0.5)(-1.1, 0.5)};
\addplot[dashed,color=gray] coordinates {(1.1, -0.5)(-1.1, -0.5)};

\node[rotate=90,text width=1cm,align=center,execute at begin node=\setlength{\baselineskip}{0.1em}] at (axis cs: -1.0, 0.875) {\tiny Player 1 Translation Symmetry};
\node[rotate=0,text width=1cm,align=center,execute at begin node=\setlength{\baselineskip}{0.1em}] at (axis cs: -0.875, 1.0) {\tiny Player 2 Translation Symmetry};

\node[rotate=45,text width=5cm,align=center] at (axis cs: 0.85, 0.85) {\tiny Fold Symmetric\\[-0.9em]Player Permutation};

\node[rotate=90,text width=1cm,align=center,execute at begin node=\setlength{\baselineskip}{0.1em}] at (axis cs: -0.5, 0.875) {\tiny Player 1 Strategy Permutation};
\node[rotate=0,text width=1cm,align=center,execute at begin node=\setlength{\baselineskip}{0.1em}] at (axis cs: -0.875, 0.5) {\tiny Player 2 Strategy Permutation};

==> tex/part_quadrant_names.tex <==
% Quadrants.
\node[text width=6.5cm,align=center] at (axis cs: -0.5, 1.06) {\scriptsize Anti-Clockwise Cyclic\\[-0.5em] Invariant-Zero-Sum Quadrant};
\node[text width=6.5cm,align=center] at (axis cs: +0.5, -1.06) {\scriptsize Clockwise Cyclic\\[-0.5em] Invariant-Zero-Sum Quadrant};
\node[text width=6.5cm,align=center] at (axis cs: +0.5, 1.06) {\scriptsize Diagonal Coordination\\[-0.5em] Invariant-Common-Payoff Quadrant};
\node[text width=6.5cm,align=center] at (axis cs: -0.5, -1.06) {\scriptsize Off-Diagonal Coordination\\[-0.5em] Invariant-Common-Payoff Quadrant};


==> tex/part_symmetric_games.tex <==
% Symmetric game lines.
\addplot[dotted,color=gray] coordinates {(-1,0)(0,-1)};
\addplot[dotted,color=gray] coordinates {(1,0)(0,1)};
\addplot[dotted,color=gray] coordinates {(-1,-1)(1,1)};

\node[rotate=-45,text width=5cm,align=center] at (axis cs: -0.875 ,-0.125) {\tiny Permutation Symmetric\\[-0.9em]Games};
\node[rotate=-45,text width=5cm,align=center] at (axis cs: 0.125 ,0.875) {\tiny Permutation Symmetric\\[-0.9em]Games};
\node[rotate=45,text width=5cm,align=center] at (axis cs: -0.875 ,-0.875) {\tiny Symmetric\\[-0.9em]Games};

